When Engagement Meets Similarity: Efficient (k,r)-Core Computation on Social Networks

In this paper, we investigate the problem of (k,r)-core which intends to find cohesive subgraphs on social networks considering both user engagement and similarity perspectives. In particular, we adopt the popular concept of k-core to guarantee the engagement of the users (vertices) in a group (subgraph) where each vertex in a (k,r)-core connects to at least k other vertices. Meanwhile, we also consider the pairwise similarity between users based on their profiles. For a given similarity metric and a similarity threshold r, the similarity between any two vertices in a (k,r)-core is ensured not less than r. Efficient algorithms are proposed to enumerate all maximal (k,r)-cores and find the maximum (k,r)-core, where both problems are shown to be NP-hard. Effective pruning techniques significantly reduce the search space of two algorithms and a novel (k,k')-core based (k,r)-core size upper bound enhances performance of the maximum (k,r)-core computation. We also devise effective search orders to accommodate the different nature of two mining algorithms. Comprehensive experiments on real-life data demonstrate that the maximal/maximum (k,r)-cores enable us to find interesting cohesive subgraphs, and performance of two mining algorithms is significantly improved by proposed techniques.

==> adaptive.tex <==
\section{Adaptive Solution}
\label{sec:adaptive}

\subsection{Motivation}
\label{subsec:ada_motivation}


\subsection{Adaptive Algorithm}
\label{subsec:ada_alg}

\begin{algorithm}[htb]
\SetVline % save space
\SetFuncSty{textsf}
\SetArgSty{textsf}
\small
\caption{\bf AdaptiveSearch($M$, $C$, $E$)}
\label{alg:adaptive}
\Input
{
   $M :$ vertices chosen, $C :$ candidate vertices, \\
   $E :$ relevant excluded vertices
}
\Output{report the identified maximal \krc}
\If{ Update($M$, $C$, $E$)}
{
	\If{$\eta(C) \leq r$ }
	{
		\State{Output $M~\cup~C$ \textit{If} \textbf{CheckMaximal}($M~\cup~C$)}
	}
	\Else
	{
	
		\State{ $u \leftarrow$ a vertex in $C$ used for expansion or shrink}
		\If { Expansion is prefered }
		{
			\State{\textbf{AdaptiveSearch}($M \cup u$, $C \setminus u$, $E$)}
		    \State{\textbf{AdaptiveSearch}($M$, $C \setminus u$, $E \cup u$)}
		}	
		\Else
		{
			\State{\textbf{AdaptiveSearch}($M$, $C \setminus u$, $E \cup u$)}
			\State{\textbf{AdaptiveSearch}($M \cup u$, $C \setminus u$, $E$)}		    	
		}
	}
}
\end{algorithm}

\begin{algorithm}[htb]
\SetVline % save space
\SetFuncSty{textsf}
\SetArgSty{textsf}
\small
\caption{\bf Update($M$, $C$, $E$)}
\label{alg:updateAd}
\Input
{
   $M :$ vertices chosen, $C :$ candidate vertices, \\
   $E :$ relevant excluded vertices
}
\Output{Refined $M$, $C$ and $E$}
\If{ Update is invoked by the insertion of $u$ }
{
	\State{Remove vertices $\{v\}$ from $C$ with $\delta(u,v) > r$ }
	\State{Remove vertices $\{v\}$ from $E$ with $\delta(u,v) > r$ }
}
% add critical points of C in M
\State{$T \leftarrow \emptyset$}	
\For{ each vertex $u \in M$ with $deg(u, M\cup C)= k$ and $deg(u,M) < k$}
{
	\State{$T \leftarrow $ $T \cup N(u, C \cup u )$}
}
\If {$\eta(T) > r$}
{
	\Return{$false$;}
}
\Else
{
	\State{ $M:= M \cup T$; $C:= C \setminus T$}
}
\State{$L, E \leftarrow$ k-core($M \cup C$)} 	
\If{$M \subseteq L$}
{
	\State{ $C:= L \setminus M$ }	
	% find early terminate points in E ?
	\If{ Find a vertex $u \in E$ s.t. $deg(u,M \cup u)\geq k$ and $\delta_{max}(u,C) \leq r$ }
	{
		\Return{$false$;}
	}
	\Else
	{
		% find early insertion points in C
		\For{ each vertex $u \in C$ with $deg(u,M \cup u) \geq k$ and $\delta_{max}(u,C) \leq r$ }
		{
			\State{$M := M \cup u$; $C := C \setminus u$}
		}
		\Return{$true$;}
	}
}
\Else
{
	\Return{$false$;}
}
\end{algorithm}


==> bk.tex <==
\section{Preliminaries}
\label{sec:preli}
In this section, we first formally introduce the concept of \krc.
Then we show the problem of enumerating all \krcs is NP-hard. Table~\ref{tb:notations} summarizes the mathematical notations used throughout this paper.
\begin{table}
  \centering
    \begin{tabular}{|c|l|}
      \hline
      % after   			\\: \hline or \cline{col1-col2} \cline{col3-col4} ...
      \textbf{Notation}   & \textbf{Definition}                   \\ \hline \hline
      $\delta(u,v)$  & similarity/distance between two vertices \\ 
                     &  $u$ and $v$  \\ \hline
    \end{tabular}
%\vspace{-2mm}
\caption{The summary of notations}
\label{tb:notations}
\vspace{-2mm}
\end{table}


\subsection{Problem Definition}
\label{subsec:prob}
We consider an undirected, unweighted, simple attribute graph $G=(V,E,A)$, where $V(G)$ ($E(G)$) represents the set of vertices (edges) in $G$ and $A(G)$ denote the attribute of the vertices. By $\delta(u,v)$, we denote the similarity/distance\footnote{
Throughout this paper, we might use similarity and distance interchangeably and appropriately chosen for better understanding of the idea.}
of two vertices $u$, $v$ in $V(G)$ which is derived based on their corresponding attribute values (e.g., user's location or user's hobbies). 
In this paper, we assume $\delta(u,v)$ is a metric distance which covers most of the popular similirity measurements such as Eucledean distance, Jaccard similarity and Edit distance.

We use $S \subseteq G$ to denote that $S$ is a \textit{induced subgraph} of $G$ where $V(S)=S$, $E(S) \subseteq E(G)$ and 
$A(S) \subseteq A(G)$. For each vertex $u \in S$, we use $N(u,S)$ to denote the set of neighbors of $u$ in $S$
and $d(u,S)$ represents $|N(u,S)|$, i.e., the number of vertices in $N(u,S)$.  
When the context is clear, they are abbreviated as $N(u)$ and $d(u)$, respectively. 

Now we formally introduce two contraints, namely \textit{connectivity constraint} and \textit{similiarity constraint}, 
which describe the cohesiveness of the vertices in a graph from graph structure and attributes perspectives, respectively.

\vspace*{0.1cm}
\begin{definition} \textbf{Connectivity Constraint.}
Given an integer $k > 0$, we say a subgraph $S$ satisfies the connectivity constraint if $d(u,S) \geq k$
for any vertex $u \in V(S)$.
\end{definition}

Without loss of generality, we assume the smaller distance/similarity value is prefered in this paper since 
Eucledean distance is used in our running examples. 

\vspace*{0.1cm}
\begin{definition} \textbf{Similarity Constraint.} 
Given a similarity threshold $r$, we say a subgraph $S$ satisfies the similarity constraint 
if $\delta(u,v) \leq r$ for any two vertices $u$, $v$ in $V(S)$.
\end{definition}

Besides the connectivity and similarity constraints, we also enforce that the cohensive subgraph
is a connected graph. 
Below is the formal definition of \krc.

\vspace*{0.1cm}
\begin{definition} \textbf{\krc.} 
Given a connected subgraph $S \subseteq G$, we say $S$ is a \krc if $S$ satisfies both connectivity and similarity constraints.
\end{definition}

In this paper, we are only interested in the \textbf{maximal} \krc;  
that is, $S$ is a \krc of $G$ and there exists no \krc $S'$ of $G$ such that $S \subset S'$.

\vspace*{2mm}
\noindent \textbf{Problem Statement}.
Given an attribute graph $G$, an integer $k$ and a similarity threshold $r$, we aim to efficiently enumerate all \textbf{maximal} \textbf{\krcs} in $G$.

\begin{example}
 
\end{example}
% \vspace*{0.2cm}
% In geo-social networks, each vertex and each edge in the graph $G$ represents a user and a friend relationship respectively. One general case of vertex attribute is location, in which similarity is geographical distance between a pair of vertices. Obviously, \textit{k-constraint} is the structure constraint and \textit{r-constraint} is the similarity constraint. Therefore, \textit{(k,r)-core} is a cohesive subgraph i.e., a community with close friendship and near geographic distance among members. Another attribute case could be keywords, in which similarity is matching degree of a pair of keywords set. Therefore, \textit{(k,r)-core} is a cohesive subgraph i.e., a community with close friendship and high correlation among members.

\subsection{Problem Hardness}
\label{subsec:hardness}
We shows that the problem studied in this paper is NP-hard based on the maximal clique problem.
\begin{theorem}
\label{the:hardness}
The problem of finding maximal \krcs is NP-hard.
\end{theorem}
\begin{proof}
Given a graph $G(V,E)$, we construct an attribute graph $G'(V',E',A)$ as follows.
We have $V(G') = V(G)$ and $G'$ is a complete graph, i.e., $(u,v) \in E(G')$ for any two vertices $u$ and $v \in V(G')$. 
Let attribute of each vertex in $V(G')$ be a set. 
More specifically,  $A(u) = \{ e \}$ for each $u \in V(G')$ where $e$ is an edge connected to $u$ in $E(G)$, 
i.e., $A(u) = \{(u,v)| (u,v) \in E(G) $ for any vertex $v \in V(G')$ $\}$.
Suppose the Jaccard similarity is employed and we set $\delta(u,v) = -\frac{|A(u)\cap A(v)|}{|A(u) \cup A(v)|}$ for
vertices $u$ and $v$ in $V(G')$ because we assume the smaller value is preferred in this paper.
Let similarity threshold $r = - \epsilon$ where $\epsilon$ is an infinite small positive number,
we have $\delta(u,v) \leq r$ if the edge $(u,v) \in E(G)$, and otherwise $\delta(u,v)=0 > r$. 
Since $G'$ is a complete graph, i.e., any subgraph $S \subseteq G'$ with $|S| \geq k$ satisfies the connectivity constraint, 
the problem of enumerating maximal $k$ cliques on $G$ can be reduced to the problem of finding maximal \krcs on $G'$ with $r = -\epsilon$. 
Consequently, Theorem~\ref{the:hardness} holds due to the NP-hardness of the maximal $k$ cliques problem~\cite{}.
\end{proof}


==> command.tex <==
\newcounter{example}[section]
\renewcommand{\theexample}{\nthesection.\arabic{example}}
\newenvironment{example}{
     \refstepcounter{example}
     {\vspace{0ex} \noindent\bf  Example  \theexample:}}{
     \eop\vspace{0ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcounter{definition}[section]
\renewcommand{\thedefinition}{\nthesection.\arabic{definition}}
\newenvironment{definition}{
     \refstepcounter{definition}
     {\vspace{0ex} \noindent\bf  Definition  \thedefinition:}}{
     \eop\vspace{0ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcounter{theorem}[section]
\renewcommand{\thetheorem}{\nthesection.\arabic{theorem}}
\newenvironment{theorem}{\begin{em}
        \refstepcounter{theorem}
        {\vspace{0ex} \noindent\bf  Theorem  \thetheorem:}}{
        \end{em}\eop\vspace{0ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcounter{lemma}[section]
\renewcommand{\thelemma}{\nthesection.\arabic{lemma}}
\newenvironment{lemma}{\begin{em}
        \refstepcounter{lemma}
        {\vspace{0ex}\noindent\bf Lemma \thelemma:}}{
        \end{em}\eop\vspace{0ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcounter{remark}[section]
\renewcommand{\theremark}{\nthesection.\arabic{remark}}
\newenvironment{remark}{\begin{em}
        \refstepcounter{remark}
        {\vspace{0ex}\noindent\bf Remark \theremark:}}{
        \end{em}\eop\vspace{0ex}} %\hspace*{\fill}\vspace*{1ex}}


\newcommand{\proofsketch}{\noindent{\bf Proof Sketch: }}
\newcommand{\myproof}{\noindent{\bf Proof: }}
% \newcommand{\proof}{\noindent{\em Proof: }}

\newcommand{\nthesection}{\arabic{section}}
% \newcommand{\thetheorem}{\thesection.\arabic{theorem}}


% End of proof
\newcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}}
% \renewcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}\vspace*{1ex}}

% Small Title
\newcommand{\stitle}[1]{\vspace{0ex} \noindent{\underline{\bf #1}}}

\newcommand{\sstitle}[1]{\vspace{0ex} \noindent{\textit{ #1}}}
\newcommand{\ssstitle}[1]{\vspace{0ex} \noindent{\textbf{ #1}}}

\newcommand{\kw}[1]{{\ensuremath {\mathsf{#1}}}\xspace}
\newcommand{\bkw}[1]{{\ensuremath {\mathsf{\textbf{#1}}}}\xspace}

\newcommand{\kwnospace}[1]{{\ensuremath {\mathsf{#1}}}}
\newcommand{\ltt}{\kw{LTT}}
\newcommand{\arr}{\kw{arrive}}
\newcommand{\vp}{\kw{p}}

\newcommand{\bellf}{{\sc Bellman-Ford}\xspace}
\newcommand{\bfalgo}{{\sc OR}\xspace}

\newcommand{\aalgo}{{\sc KDXZ}\xspace}

\newcommand{\dijk}{{\sc Dijkstra}\xspace}
%\newcommand{\dalgo}{{\sc DLY}\xspace}
\newcommand{\dalgo}{{\sc Two-Step-LTT}\xspace}

\newcommand{\dtalgo}{{\sc DOT}\xspace}


\newcommand{\genfunc}{{\sl timeRefinement}\xspace}
\newcommand{\pathc}{{\sl pathSelection}\xspace}
\newcommand{\fifo}{{\sl FIFO}\xspace}

\newcommand{\st}{starting time\xspace}
\newcommand{\sti}{starting-time interval\xspace}
\newcommand{\stsi}{starting-time subinterval\xspace}
\newcommand{\stsis}{starting-time subintervals\xspace}
\newcommand{\stis}{starting-time intervals\xspace}
\newcommand{\ti}{time interval\xspace}
\newcommand{\tis}{time intervals\xspace}
\newcommand{\ttime}{travel time\xspace}
\newcommand{\ttimea}{travel time\xspace}
\newcommand{\at}{arrival time\xspace}
\newcommand{\ata}{arrival-time\xspace}
\newcommand{\atf}{arrival-time function\xspace}
\newcommand{\ati}{arrival-time interval\xspace}
\newcommand{\ats}{arrival times\xspace}
\newcommand{\ed}{edge delay\xspace}
\newcommand{\eda}{edge-delay\xspace}
\newcommand{\edf}{edge-delay function\xspace}
\newcommand{\eds}{edge delays\xspace}
\newcommand{\wt}{waiting time\xspace}

\newcommand{\g}{\overline{g}}
\newcommand{\iend}{\tau}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Defined in XML Paper %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\myhead}[1]{\vspace{.05in} \noindent {\bf #1.}~~}
\newcommand{\cond}[1]{(\emph{#1})~}
\newcommand{\op}[1]{(\emph{#1})~}

\newcommand{\qc}{\ensuremath{Q^c}}


\newcommand{\rewrite}{\kw{XPathToReg}}

\newcommand{\upparen}[1]{\ensuremath{\mathrm{(}}{#1}\ensuremath{\mathrm{)}}}
\newcommand{\func}[2]{\funcname{#1}\upparen{\ensuremath{#2}}}
\newcommand{\funcname}[1]{\ensuremath{\mathit{#1}}}

\newcommand\AS{\textbf{as}\ }
\newcommand{\xsltsize}{\small}

\newcommand{\X}{{\cal X}}
%\newcommand{\U}{{\cal U}}
\newcommand{\sem}[1]{[\![#1]\!]}
\newcommand{\NN}[2]{#1\sem{#2}}
\newcommand{\pcdata}{{\tt str}\xspace}

\newcommand{\exa}[2]{{\tt\begin{tabbing}\hspace{#1}\=\hspace{#1}\=\+\kill #2\end{tabbing}}}
\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\rsa}{\_} % {\rightsquigarrow}
\newcommand{\Ed}[2]{E_{{\scriptsize \mbox{#1} \rsa \mbox{#2}}}}
\newenvironment{bi}{\begin{itemize}
        \setlength{\topsep}{0.5ex}\setlength{\itemsep}{0ex}\vspace{-0.6ex}}
        {\end{itemize}\vspace{-1ex}}
\newenvironment{be}{\begin{enumerate}
        \setlength{\topsep}{0.5ex}\setlength{\itemsep}{0ex}\vspace{-0.6ex}}
        {\end{itemize}\vspace{-1ex}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ee}{\end{enumerate}}

\newcommand{\mat}[2]{{\begin{tabbing}\hspace{#1}\=\+\kill #2\end{tabbing}}}
\newcommand{\m}{\hspace{0.05in}}
\newcommand{\ls}{\hspace{0.1in}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}

\newcounter{ccc}
\newcommand{\bcc}{\setcounter{ccc}{1}\theccc.}
\newcommand{\icc}{\addtocounter{ccc}{1}\theccc.}

\newcommand{\oneurl}[1]{\texttt{#1}}
\newcommand{\tabstrut}{\rule{0pt}{4pt}\vspace{-0.1in}}
\newcommand{\tabstruct}{\rule{0pt}{8pt}\\[-2ex]}
\newcommand{\stab}{\rule{0pt}{8pt}\\[-2.2ex]}
\newcommand{\sstab}{\rule{0pt}{8pt}\\[-2.2ex]}

\newcommand{\eat}[1]{}

\newfloat{tcm}{thp}{loa}
\floatname{tcm}{Recursive \sql}

\def\subfigcapskip{2pt}
% \def\subfigtopskip{0pt}
% \def\subfigbottomskip{0pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Defined in XML Paper (END) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\rdms}{{\sc rdbms}\xspace}
\newcommand{\sql}{{\sc sql}\xspace}
\newcommand{\dbms}{{\sc dbms}\xspace}

%\newcommand{\cfig}{Figure~}
%\newcommand{\ctab}{Table~}
\newcommand{\cfig}{Fig.~}
\newcommand{\ctab}{Table~}
\newcommand{\csec}{Section~}
\newcommand{\cdef}{Definition~}
\newcommand{\cthm}{Theorem~}
\newcommand{\clem}{Lemma~}
\newcommand{\cequ}[1]{Equation~(#1)}
\newcommand{\SG}{\mathbf{SG}}
\newcommand{\SA}{\mathbf{SA}}
\renewcommand{\AA}{\mathbf{AA}}

%\newcommand{\EDA}{\textbf{EDA}}
%\newcommand{\CSP}{\textbf{CSP}}
%\newcommand{\TDSP}{\textbf{TDSP}}
%\newcommand{\SSSP}{\textbf{SSSP}}

%\newcommand{\revised}{***\texttt}
%\newcommand{\revised}{\comment}
%\newcommand{\add}{***{\texttt{ADD}}}
%\newcommand{\add}{}
%\newcommand{\add}{\comment}


\newcommand{\xml}{{\sl XML}\xspace}
\newcommand{\xlink}{{\sl XLink}\xspace}
\newcommand{\xpath}{{\sl XPath}\xspace}
\newcommand{\xpointer}{{\sl XPointer}\xspace}
\newcommand{\rdf}{{\sl RDF}\xspace}
\newcommand{\tc}{{\sl TC}\xspace}
%\newcommand{\bfs}{{\sl BFS}\xspace}
\newcommand{\dfs}{{\sl DFS}\xspace}
\newcommand{\DAG}{{\sl DAG}\xspace}
\newcommand{\DAGs}{{\sl DAG}s\xspace}
\newcommand{\grail}{{\sl GRAIL}\xspace}
\newcommand{\yesgrail}{{\sl Yes-GRAIL}\xspace}
\newcommand{\code}{\kw{code}}
\newcommand{\sit}{\kw{sit}}
\newcommand{\psit}{{\cal P}_{sit}}
\newcommand{\yescode}{{\sl Yes-Label}\xspace}
\newcommand{\nocode}{{\sl No-Label}\xspace}
\newcommand{\entry}{\kw{entry}\xspace}
\newcommand{\yngindex}{{\sl YNG-Index}\xspace}
\newcommand{\rqrun}{{\sl RQ-Run}\xspace}
\newcommand{\citeseerx}{{\sl citeseerx}\xspace}
\newcommand{\gouniprot}{{\sl go-uniprot}\xspace}
\newcommand{\uniprot}{{\sl uniprot150}\xspace}


\long\def\comment#1{}


\newcommand{\scc}{strongly connected component\xspace}
\newcommand{\sccs}{strongly connected components\xspace}
\newcommand{\sscc}{\kw{SCC}}
\newcommand{\ssccs}{\kwnospace{SCC}s\xspace}
\newcommand{\sccg}{\kwnospace{SCC}\textrm{-}\kw{Graph}}
\newcommand{\strongc}{\leftrightarrow}
\newcommand{\nstrongc}{\nleftrightarrow}
\newcommand{\emscc}{\kwnospace{EM}\textrm{-}\kw{SCC}}
\newcommand{\dfsscc}{\kwnospace{DFS}\textrm{-}\kw{SCC}}
\newcommand{\dfstree}{\kwnospace{DFS}\textrm{-}\kw{Tree}}
%\newcommand{\len}{\kw{length}}
\newcommand{\len}{\kw{len}}
\newcommand{\dep}{\kw{depth}}
% \newcommand{\tdep}{\kw{mdepth}}
% \newcommand{\tlink}{\kw{mnode}}
\newcommand{\tdep}{\kw{drank}}
\newcommand{\tlink}{\kw{dlink}}
\newcommand{\vedges}{up-edges\xspace}
\newcommand{\vedge}{up-edge\xspace}
% \newcommand{\dedges}{down-edges\xspace}
% \newcommand{\dedge}{down-edge\xspace}
\newcommand{\cvedge}{Up-Edge\xspace}

\newcommand{\drsscc}{\kwnospace{1P}\textrm{-}\kw{SCC}}
\newcommand{\drssccb}{\kwnospace{1PB}\textrm{-}\kw{SCC}}


\newcommand{\Bdrsscc}{\kwnospace{B}\textrm{-}\kwnospace{BR'}\textrm{-}\kw{SCC}}


\newcommand{\deprtree}{depth-ranked tree\xspace}
\newcommand{\cdeprtree}{Depth-Ranked Tree\xspace}
\newcommand{\drtree}{\kwnospace{BR}\textrm{-}\kw{Tree}}
\newcommand{\drplustree}{\kwnospace{BR}$^+$\textrm{-}\kw{Tree}}
\newcommand{\drscc}{\kwnospace{2P}\textrm{-}\kw{SCC}}
\newcommand{\updatedrank}{\kwnospace{update}\textrm{-}\kw{drank}}

%\newcommand{\drtreeconstruct}{\kwnospace{BR}\textrm{-}\kwnospace{Tree}\textrm{-}\kw{Construction}}
%\newcommand{\drtreesearch}{\kwnospace{BR}\textrm{-}\kwnospace{Tree}\textrm{-}\kw{Search}}
\newcommand{\drtreeconstruct}{\kwnospace{Tree}\textrm{-}\kw{Construction}}
\newcommand{\drtreesearch}{\kwnospace{Tree}\textrm{-}\kw{Search}}
%\newcommand{\depthrerank}{\kwnospace{depth}\textrm{-}\kw{rerank}}
\newcommand{\depthrerank}{\kw{pushdown}}
\newcommand{\itrerank}{\kwnospace{iterative}\textrm{-}\kw{rerank}}
\newcommand{\drr}{\Downarrow}
\newcommand{\reach}{\kw{Rset}}
\newcommand{\earlyrejection}{\kwnospace{early}\textrm{-}\kw{rejection}}
\newcommand{\earlyacceptance}{\kwnospace{early}\textrm{-}\kw{acceptance}}
%\newcommand{\greduce}{\kwnospace{graph}\textrm{-}\kw{reduction}}
\newcommand{\greduce}{\earlyacceptance}
\newcommand{\drea}{\kwnospace{1P}\textrm{/}\kw{ER}}
\newcommand{\myinf}{\kw{INF}}

%==========defined in GCloud ========
\newcommand{\gcloud}{\kw{GCloud}\xspace}
\newcommand{\degree}{\kw{Degree}\xspace}
\newcommand{\subgraph}{\kw{Subgraph}\xspace}
\newcommand{\pagerank}{\kw{PageRank}\xspace}
\newcommand{\bfs}{\kw{BFS}\xspace}
\newcommand{\keysearch}{\kw{KWS}\xspace}
\newcommand{\cc}{\kw{CC}\xspace}
\newcommand{\msf}{\kw{MSF}\xspace}
\newcommand{\dmax}{\kw{rmax}}
\newcommand{\mystar}{\kw{star}\xspace}
\newcommand{\twitter}{{\sl{Twitter-2010}}\xspace}
\newcommand{\friendster}{{\sl{Friendster}}\xspace}
\definecolor{lgray}{gray}{0.85}
\definecolor{llgray}{gray}{0.9}
\newcommand{\mycc}{CC\xspace}
\newcommand{\myccs}{CCs\xspace}
\newcommand{\mymsf}{MSF\xspace}
\newcommand{\oneroundmsf}{\kw{OneRoundMSF}}
\newcommand{\multiroundmsf}{\kw{MultiRoundMSF}}

\newcommand{\hashtomin}{\kw{HashToMin}\xspace}
\newcommand{\hashgreatertomin}{\kw{HashGToMin}\xspace}
\newcommand{\pramsimulation}{\kwnospace{PRAM}\textrm{-}\kw{Simulation}\xspace}

\newcommand{\pagerankpig}{\kwnospace{PageRank}\textrm{-}\kw{Pig}\xspace}
\newcommand{\bfspig}{\kwnospace{BFS}\textrm{-}\kw{Pig}\xspace}
\newcommand{\keysearchpig}{\kwnospace{KWS}\textrm{-}\kw{Pig}\xspace}

%=============defined in SubgEnum======
\newcommand{\ttwig}{\kwnospace{TwinTwig}\xspace}
\newcommand{\ttwigs}{\kwnospace{TwinTwig}s\xspace}
\newcommand{\ttjoin}{\kwnospace{TwinTwig}\kw{Join}}
\newcommand{\sdec}{\kwnospace{SDEC}\xspace}
\newcommand{\subgenum}{\kwnospace{SubgraphEnum}\xspace}
\newcommand{\mymap}{\kwnospace{map}\xspace}
\newcommand{\myreduce}{\kwnospace{reduce}\xspace}
\newcommand{\cascadejoin}{\kwnospace{Edge}\kw{Join}}
\newcommand{\starjoin}{\kwnospace{Star}\kw{Join}}
\newcommand{\multiwayjoin}{\kwnospace{Multiway}\kw{Join}}
\newcommand{\cost}{\kwnospace{cost}\xspace}
\newcommand{\mysize}{\kwnospace{card}\xspace}
%\newcommand{\auto}{\kwnospace{auto}\xspace}
\newcommand{\er}{\kwnospace{ER}\xspace}
\newcommand{\optdec}{\kwnospace{Optimal}\textrm{-}\kwnospace{Decomp}\xspace}


\newcommand{\ttone}{\kwnospace{TT1}\xspace}
\newcommand{\tttwo}{\kwnospace{TT2}\xspace}
\newcommand{\ttthree}{\kwnospace{TT3}\xspace}


\newcommand{\alEdge}{\kwnospace{Edge}\xspace}
\newcommand{\alMul}{\kwnospace{Mul}\xspace}
\newcommand{\alStar}{\kwnospace{Star}\xspace}

%\newcommand{\alTTBO}{\kwnospace{TTBO}\xspace}
%\newcommand{\alTTNLB}{\kwnospace{TTNLB}\xspace}
%\newcommand{\alTTLB}{\kwnospace{TTLB}\xspace}
%\newcommand{\alTTFil}{\kwnospace{TTFil}\xspace}

\newcommand{\alTTBO}{\kwnospace{TTBS}\xspace}
\newcommand{\alTTNLB}{\kwnospace{TTOA}\xspace}
\newcommand{\alTTLB}{\kwnospace{TTLB}\xspace}
\newcommand{\alTTFil}{\kwnospace{TT}\xspace}


%=============defined for reference======
\newcommand{\reffig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\refsec}[1]{Section~\ref{sec:#1}}
\newcommand{\reftable}[1]{Table~\ref{tab:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{alg:#1}}
\newcommand{\refeq}[1]{Eq.~\ref{eq:#1}}
\newcommand{\refdef}[1]{Definition~\ref{def:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{thm:#1}}
\newcommand{\reflem}[1]{Lemma~\ref{lem:#1}}
\newcommand{\refex}[1]{Example~\ref{ex:#1}}

\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

%===============defined for DivKClique======
\newcommand{\enumall}{\kwnospace{Enum}\kw{All}}
\newcommand{\enumsub}{\kwnospace{Enum}\kw{Sub}}
\newcommand{\cliqueall}{\kwnospace{Clique}\kw{All}}
\newcommand{\cliquesub}{\kwnospace{Clique}\kw{Sub}}
\newcommand{\maxcover}{\kwnospace{Max}\kw{Cover}}
\newcommand{\enumk}{\kwnospace{Enum}\kw{K}}
\newcommand{\priv}{\kw{priv}}
\newcommand{\cov}{\kw{cov}}
\newcommand{\enumkbasic}{\kwnospace{Enum}\kwnospace{K}\kw{Basic}}
\newcommand{\enumkopt}{\kwnospace{Enum}\kwnospace{K}\kw{Opt}}
\newcommand{\candmaintainbasic}{\kwnospace{Cand}\kwnospace{Maintain}\kw{Basic}}
\newcommand{\candmaintain}{\kwnospace{Cand}\kw{Maintain}}
\newcommand{\pnpindex}{\kwnospace{PNP}\textrm{-}\kw{Index}}
\newcommand{\rcov}{\kw{rcov}}
\newcommand{\rpriv}{\kw{rpriv}}
\newcommand{\insertc}{\kw{Insert}}
\newcommand{\deletec}{\kw{Delete}}
\newcommand{\calp}{\kwnospace{Cal}\kw{P}}

\newcommand{\myscore}{\kw{score}}
\newcommand{\initk}{\kw{InitK}}
\newcommand{\globalpruning}{\kw{GlobalPruning}}
\newcommand{\localpruning}{\kw{LocalPruning}}
\newcommand{\cliquek}{\kw{CliqueK}}
\newcommand{\mycolor}{\kw{color}}
\newcommand{\mycore}{\kw{core}}
\newcommand{\cliquegreedy}{\kw{CliqueGreedy}}

\newcommand{\sops}{\kw{SOPS}}
\newcommand{\gops}{\kw{GOPS}}
\newcommand{\sieve}{\kw{SIEVE}}
\newcommand{\enumkglobal}{\kw{Global}}
\newcommand{\enumklocal}{\kw{Local}}

\newcommand{\dsgoogle}{\textit{Google}\xspace}
\newcommand{\dsskitter}{\textit{Skitter}\xspace}
\newcommand{\dsyoutube}{\textit{Youtube}\xspace}
\newcommand{\dspokec}{\textit{Pokec}\xspace}
\newcommand{\dswiki}{\textit{Wiki}\xspace}
\newcommand{\dsuk}{\textit{UK-2002}\xspace}



==> conclusion.tex <==
\section{Conclusion}
\label{sec:con}
In this paper, we propose a novel cohesive subgraph model, called \krc,
which considers the cohesiveness of a subgraph from the perspective of both graph structure and vertex attribute.
We show that the problem of enumerating the maximal \krcs and finding the maximum \krc are both NP-hard.
Several novel pruning techniques are proposed to improve algorithm efficiency,
including candidate size reduction, early termination, checking maximals and upper bound estimation techniques.
We also devise effective search orders for enumeration, maximum and maximal check algorithms.
Extensive experiments on real-life networks demonstrate the effectiveness of the \krc model, as well
as the efficiency of our techniques.


==> expansion_shrink.tex <==

\subsection{Expansion Based Approach}
\label{subsec:expansion}

\begin{algorithm}[htb]
\SetVline % save space
\SetFuncSty{textsf}
\SetArgSty{textsf}
\small
\caption{\bf Expand($M$, $C$)}
\label{alg:expand}
\Input
{
   $M :$ vertices already chosen, \\
   $C :$ candidate vertices to be inserted
}
\Output{Return true if we find a \krc}
\If{ $C = \emptyset$ }
{
	\State{Output $M~\cup~C$ \textit{If} \textbf{CheckMaximal}($M~\cup~C$) }
    \Return{$true$;}
}
\Else
{
    \State{ $F := false$ }
	\For {each vertex $u \in C$}
	{
		\State{$C' :=$ \{ $v$~$|$~$v \in C$ and $\delta(u,v) \leq r$ \} }
		\State{$L :=$ k-core($M \cup C'$, $k$)}
		\If{ $M \cup u \subseteq L$ }
		{
			\State{$C'$ $:= L$ $\setminus$ ($M \cup u$)}
			\State{$F:= true$ \textbf{If} Expand($M~\cup~u$, $C'$)}
		}
		\State{$C = C \setminus u$}
	}
    \If {$F=false$ and $d_{min}(M) \geq k$ }
    {
         \Return{Expand($M$, $\emptyset$);}
     }
    \Else
    {
        \Return{$false$;}    
    }      
}
\end{algorithm}


\subsection{Shrink Based Approach}
\label{subsec:shrink}

\begin{algorithm}[htb]
\SetVline % save space
\SetFuncSty{textsf}
\SetArgSty{textsf}
\small
\caption{\bf Shrink($M$, $C$)}
\label{alg:shrink}
\Input
{
   $M :$ vertices must be included, \\
   $C :$ candidate vertices to be removed
}
\Output{ report the identified maximal \krc}
\If{$\eta(M~\cup~C) \leq r$ }
{
	\State{Output $M~\cup~C$ \textit{If} \textbf{CheckMaximal}($M~\cup~C$)}
}
\Else
{
    	\For {each vertex $u \in C$}
    	{
    		\State{$C' := C \setminus u$}
    		\State{$L :=$ k-core($M \cup C'$, $k$)}
    		\If{ $M \subseteq L$ }
    		{
    			\State{$C'$ $:= L$ $\setminus$ ($M$)}
    			\State{Shrink($M$, $C'$)}
    		}
    		\State{$M = M \cup u$}
			\If {$\eta(M) > r$ }
			{
		      	\Return{;}
			}
    	}
}
\end{algorithm}

==> temp.tex <==
\vspace{-0.1mm}
\noindent \textbf{(1) \underline{Candidate size}}. We develop effective structural and similarity based pruning techniques to reduce the 
candidate size, and hence shorten the height of the search tree.

\vspace{-0.1mm}
\noindent \textbf{(2) \underline{Early termination}}. The maximal property of the result enables us to terminate the search of a subtree if we can predict that all possible \krcs derived in the subtree are not maximal. 

\vspace{-0.1mm}
\noindent \textbf{(3) \underline{Maximal Check}}. To deal with possibly large number of \krcs, we also develop novel algorithm to avoid checking maximal property against all solutions. Regarding the maximum \krc, it is critical to estimate the maximal size of the solutions in a subtree such that we can cut off the non-promising subtrees according to maximal size of the \krcs seen so far.

\textit{early termination},
\textit{maximal check}, \textit{upper bound} of core size, and \textit{visiting order}.
Particularly, we develop effective structural and similarity based pruning techniques to reduce the 
candidate size, and hence shorten the height of the search tree. 
The maximal property of the result enables us to terminate the search of a subtree if we can predict that all possible \krcs derived in the subtree are not maximal.
To deal with possibly large number of \krcs, we also develop novel algorithm to avoid checking maximal property against all solutions.
Regarding the maximum \krc, it is critical to estimate the maximal size of the solutions in a subtree such that 
we can cut off the non-promising subtrees according to maximal size of the \krcs seen so far.


Our empirical study shows that the visiting order of the algorithms is crutial to the performance.
A bad choice of the order may result in very poor performance, even all of other advanced techniques are applied.
Based on some key observations, three effective visiting order strategies are proposed for 
enumeration, finding maximal, and maximal check algorithms according to their different nature.



\noindent \textbf \underline{Candidate size}, \textit{early termination},
\textit{maximal check}, \textit{upper bound} of core size, and \textit{visiting order}.
Particularly, we develop effective structural and similarity based pruning techniques to reduce the 
candidate size, and hence shorten the height of the search tree. 
The maximal property of the result enables us to terminate the search of a subtree if we can predict that all possible \krcs derived in the subtree are not maximal.
To deal with possibly large number of \krcs, we also develop novel algorithm to avoid checking maximal property against all solutions.
Regarding the maximum \krc, it is critical to estimate the maximal size of the solutions in a subtree such that 
we can cut off the non-promising subtrees according to maximal size of the \krcs seen so far.
In this paper, we develop novel ($k$, $k'$)-core method to estimate the size upper bound of the cores 
in an interactively way from the structural and similarity perspectives. 
Our empirical study shows that the visiting order of the algorithms is crutial to the performance.
A bad choice of the order may result in very poor performance, even all of other advanced techniques are applied.
Based on some key observations, three effective visiting order strategies are proposed for 
enumeration, finding maximal, and maximal check algorithms according to their different nature.
